Learning Goal-Oriented Visual Dialog Agents: Imitating and Surpassing Analytic Experts

This paper tackles the problem of learning a questioner in the goal-oriented visual dialog task. Several previous works adopt model-free reinforcement learning. Most pretrain the model from a finite set of human-generated data. We argue that using limited demonstrations to kick-start the questioner is insufficient due to the large policy search space. Inspired by a recently proposed information theoretic approach, we develop two analytic experts to serve as a source of high-quality demonstrations for imitation learning. We then take advantage of reinforcement learning to refine the model towards the goal-oriented objective. Experimental results on the GuessWhat?! dataset show that our method has the combined merits of imitation and reinforcement learning, achieving the state-of-the-art performance.

==> tables/accuracy_old.tex <==

\begin{table*}[ht]
\caption{The game success rates (in percentage) of our model on GuessWhat?!. ``NO'' stands for ``New objects,'' referring to uniformly sampling target objects in training data whereas ``NP'' means ``new pictures,'' referring to the fixed test set. For ``new objects'', we run the model 5 times and report the mean. Numbers are highlighted in boldface when our scheme outperforms IGE.} 
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|cccc|cccc|cccc|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{4}{c|}{trueA} & \multicolumn{4}{c|}{depA} & \multicolumn{4}{c|}{indA} & \multirow{2}{*}{Strub et al.~\cite{end_to_end_gw}} & \multirow{2}{*}{Zhao et al.~\cite{Zhao2018ImprovingGV}} & \multirow{2}{*}{Human~\cite{end_to_end_gw}} \\ \cline{3-14}
\multicolumn{2}{|c|}{} & 3q & 5q & 8q & 10q & 3q & 5q & 8q & 10q & 3q & 5q & 8q & 10q &  &  &  \\ \hline
\multirow{2}{*}{NO} & Ours & 62.31 & 71.53 & 82.07 & \textbf{83.84} & 58.45 & 70.70 & 80.49 & \textbf{82.02} & 56.48 & 68.87 & \textbf{76.47} & \textbf{78.20} & \multirow{2}{*}{60.3} & \multirow{2}{*}{-} & \multirow{5}{*}{84.4} \\ %\cline{2-2}
 & IGE & 73.31 & 81.34 & 83.13 & 83.48 & 72.38 & 79.15 & 80.58 & 80.88 & 66.03 & 71.50 & 72.65 & 72.89 &  &  &  \\ \cline{1-16}
\multirow{3}{*}{NP} & Ours & 60.18 & 69.32 & 80.96 & \textbf{82.45} & 55.73 & 68.65 & 79.13 & \textbf{80.68} & 54.26 & 66.95 & \textbf{74.85} & \textbf{76.31} & \multirow{3}{*}{58.4} & \multirow{3}{*}{74.31} &  \\ %\cline{2-2}
 & IGE & 70.71 & 80.0 & 81.79 & 82.24 & 70.23 & 78.58 & 79.44 & 79.71 & 63.91 & 69.77 & 71.15 & 71.43 &  &  &  \\ %\cline{2-2}
 & AQM~\cite{NIPS2018_7524} & 63.76 & - & - & 81.96 & - & 72.89 & - & 78.72 & - & 66.73 & - & - &  &  &  \\ \hline
\end{tabular}%
}


\label{tab:acc}
\end{table*}


